Equilibrium Computation in Multi-Stage Auctions and Contests

We compute equilibrium strategies in multi-stage games with continuous signal and action spaces as they are widely used in the management sciences and economics. Examples include sequential sales via auctions, multi-stage elimination contests, and Stackelberg competitions. In sequential auctions, analysts performing equilibrium analysis are required to derive not just single bids but bid functions for all possible signals or values that a bidder might have in multiple stages. Due to the continuity of the signal and action spaces, these bid functions come from an infinite dimensional space. While such models are fundamental to game theory and its applications, equilibrium strategies are rarely known. The resulting system of non-linear differential equations is considered intractable for all but elementary models. This has been limiting progress in game theory and is a barrier to its adoption in the field. We show that Deep Reinforcement Learning and self-play can learn equilibrium bidding strategies for various multi-stage games. We find equilibrium in models that have not yet been explored analytically and new asymmetric equilibrium bid functions for established models of sequential auctions. The verification of equilibrium is challenging in such games due to the continuous signal and action spaces. We introduce a verification algorithm and prove that the error of this verifier decreases when considering Lipschitz continuous strategies with increasing levels of discretization and sample sizes.

==> tables/table_sequential_auction_interdependent.tex <==
\begin{table}
\centering
\caption{Final approximated utility losses of the experiments with valuation interdependencies.}
\label{tab:table_sequential_auction_interdependent}
\begin{tabular}{lllrr}
	\toprule
	mechanism & $T$ & metric & \textsc{Reinforce}  &    PPO        \\
	\midrule
	% first & 1 & $L_2^{S1}$ &    0.0143 (0.0016) &  0.0065 (0.0016) \\ \cdashline{3-5}
	first & 1 & $\ell$ &    0.0001 (0.0002) &     0.0000 (0.0002) \\ \cdashline{3-5}
	&   & $\ell^\text{est}$ &          0.0000 (0.0000) &    -0.0001 (0.0000) \\ \cdashline{2-5}
	& 2 & $\ell^\text{est}$ &    0.0004 (0.0001) &    0.0000 (0.0001) \\ \hline
	% second & 1 & $L_2^{S1}$ &    0.0098 (0.0011) &  0.0065 (0.0021) \\ \cdashline{3-5}
	second & 1 & $\ell$ &    0.0001 (0.0001) &    0.0000 (0.0002) \\ \cdashline{3-5}
	&   & $\ell^\text{est}$ &         0.0000 (0.0000) &       0.0000 (0.0000) \\ \cdashline{2-5}
	& 2 & $\ell^\text{est}$ &    0.0011 (0.0008) &  0.0024 (0.0015) \\
	\bottomrule
\end{tabular}
\end{table}


==> tables/table_sequential_auction_risk.tex <==
\begin{table}
\centering
\caption{Final approximated utility losses of the experiments with risk averse bidders.}
\label{tab:table_sequential_auction_risk}
\begin{tabular}{lllrr}
\toprule
mechanism & risk $\rho$ & metric & \textsc{Reinforce} &           PPO  \\
\midrule
first & 0.25 & $\ell^\text{est}$ &    0.0009 (0.0002) &  0.0003 (0.0001) \\ \cdashline{2-5}
       & 0.50 & $\ell^\text{est}$ &     0.0010 (0.0002) &  0.0005 (0.0002) \\ \cdashline{2-5}
       & 0.75 & $\ell^\text{est}$ &    0.0011 (0.0002) &  0.0007 (0.0003) \\ \cdashline{2-5}
       & 1.00 & $\ell^\text{est}$ &    0.0013 (0.0002) &  0.0004 (0.0004) \\ \hline
second & 0.25 & $\ell^\text{est}$ &    0.0073 (0.0008) &  0.0067 (0.0004) \\ \cdashline{2-5}
       & 0.50 & $\ell^\text{est}$ &    0.0071 (0.0009) &  0.0051 (0.0009) \\ \cdashline{2-5}
       & 0.75 & $\ell^\text{est}$ &    0.0056 (0.0005) &  0.0036 (0.0008) \\ \cdashline{2-5}
       & 1.00 & $\ell^\text{est}$ &    0.0033 (0.0005) &   0.0020 (0.0006) \\
\bottomrule
\end{tabular}
\end{table}


==> tables/table_sequential_auction_symmetric_budget_constraints.tex <==
\begin{table}
\centering
\caption{Approximated utility losses in a two-stage sequential auction with affiliated values and budget constrainted bidders.}
\label{tab:table_sequential_auction_symmetric_budget_constraints}
\begin{tabular}{lllrr}
\toprule
mechanism & budget & metric &    \textsc{Reinforce}   &    PPO\\
\midrule
first-price  & 0.6 & $\ell^\text{ver}$ &    0.0058 (0.0002) &  0.0058 (0.0002) \\ \cdashline{2-5}
			 & 0.8 & $\ell^\text{ver}$ &    0.0104 (0.0002) &  0.0069 (0.0003) \\ \hline \Tstrut
second-price & 0.6 & $\ell^\text{ver}$ &    0.0045 (0.0002) &  0.0043 (0.0002) \\ \cdashline{2-5}
			 & 0.8 & $\ell^\text{ver}$ &    0.0039 (0.0001) &  0.0036 (0.0002) \\
\bottomrule
\end{tabular}
\end{table}

